Router Sensitivity Under Lightweight Fine-Tuning Identifies Prunable Experts in Mixture-of-Experts Models

Mixture-of-Experts (MoE) models decouple parameter count from per-token compute, but deployment still requires hosting every expert in memory. Recent theory shows that experts whose router weights change least during fine-tuning can be pruned with provable accuracy preservation, yet the guarantee assumes full fine-tuning. We show that the signal can be elicited through a brief parameter-efficient adaptation. We fine-tune with a lightweight adapter, rank experts by the induced router change, and prune the least-changed experts in one shot. On Mixtral-8$\times$7B-Instruct, router-only LoRA trains 0.002% of parameters and retains 27.54% MMLU-Pro accuracy with half the experts removed, against roughly 16% for magnitude and random pruning. Signal quality improves monotonically with adapter size, reaching 28.76%, and declines as adaptation spreads beyond the router. Under their shared budget, IA3 reaches 28.04% while Houlsby reaches 25.39%. The criterion transfers to Qwen1.5-MoE fine-tuned for mathematical reasoning, retaining 49.7% mean accuracy over eleven benchmarks with half the experts removed. Structural pruning reduces memory by 49% and per-token latency by 37%. Lightweight router sensitivity therefore makes provably motivated, task-conditioned expert pruning practical at scale.

==> camera_ready_layout.tex <==
% Keep the accepted submission's body layout and page breaks unchanged.
\usepackage{eso-pic}
\makeatletter
% Retain the accepted submission's line-breaking machinery, without printing
% review numbers. This avoids reflow when switching the template to final mode.
    % line numbers for submission
    \RequirePackage{lineno}
    \linenumbers

    % fix incompatibilities between lineno and amsmath, if required, by
    % transparently wrapping linenomath environments around amsmath
    % environments
    \AtBeginDocument{%
      \@ifpackageloaded{amsmath}{%
        \newcommand*\patchAmsMathEnvironmentForLineno[1]{%
          \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
          \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
          \renewenvironment{#1}%
                          {\linenomath\csname old#1\endcsname}%
                          {\csname oldend#1\endcsname\endlinenomath}%
        }%
        \newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
          \patchAmsMathEnvironmentForLineno{#1}%
          \patchAmsMathEnvironmentForLineno{#1*}%
        }%
        \patchBothAmsMathEnvironmentsForLineno{equation}%
        \patchBothAmsMathEnvironmentsForLineno{align}%
        \patchBothAmsMathEnvironmentsForLineno{flalign}%
        \patchBothAmsMathEnvironmentsForLineno{alignat}%
        \patchBothAmsMathEnvironmentsForLineno{gather}%
        \patchBothAmsMathEnvironmentsForLineno{multline}%
      }
      {}
    }

\renewcommand{\makeLineNumber}{}

% Match the original four-line author box's height and depth exactly.
\usepackage{etoolbox}
\newsavebox{\AxiomAuthorReference}
\sbox{\AxiomAuthorReference}{%
  \begin{tabular}[t]{c}\bf\rule{\z@}{24\p@}
    Anonymous Author(s) \\
    Affiliation \\
    Address \\
    \texttt{email} \\
  \end{tabular}%
}
\patchcmd{\@maketitle}
  {\begin{tabular}[t]{c}\bf\rule{\z@}{24\p@}\@author\end{tabular}}
  {\raisebox{0pt}[\ht\AxiomAuthorReference][\dp\AxiomAuthorReference]{%
    \begin{tabular}[t]{c}\bf\rule{\z@}{24\p@}\@author\end{tabular}}}
  {}{\PackageError{axiom}{Could not preserve author-box dimensions}{}}

\renewcommand{\@noticestring}{%
  \leavevmode
  \rlap{\raisebox{-10bp}[0pt][0pt]{Workshop: AXIOM, Foundations of Efficient Deep Learning.}}%
  \mbox{40th Conference on Neural Information Processing Systems (NeurIPS 2026).}%
}
\makeatother
\AddToShipoutPictureFG*{%
  \AtPageLowerLeft{%
    \setlength{\unitlength}{1bp}%
    \put(108,74){\rule{70bp}{0.4bp}}%
    \put(108,66){\fontsize{6.5bp}{8bp}\selectfont *}%
    \put(112.5,63){\fontsize{8.5bp}{10bp}\selectfont contact: aj3238@columbia.edu}%
  }%
}

